Mogao: An Omni Foundation Model for Interleaved Multi-Modal Generation

Recent progress in unified models for image understanding and generation has been impressive, yet most approaches remain limited to single-modal generation conditioned on multiple modalities. In this paper, we present Mogao, a unified framework that advances this paradigm by enabling interleaved multi-modal generation through a causal approach. Mogao integrates a set of key technical improvements in architecture design, including a deep-fusion design, dual vision encoders, interleaved rotary position embeddings, and multi-modal classifier-free guidance, which allow it to harness the strengths of both autoregressive models for text generation and diffusion models for high-quality image synthesis. These practical improvements also make Mogao particularly effective to process interleaved sequences of text and images arbitrarily. To further unlock the potential of unified models, we introduce an efficient training strategy on a large-scale, in-house dataset specifically curated for joint text and image generation. Extensive experiments show that Mogao not only achieves state-of-the-art performance in multi-modal understanding and text-to-image generation, but also excels in producing high-quality, coherent interleaved outputs. Its emergent capabilities in zero-shot image editing and compositional generation highlight Mogao as a practical omni-modal foundation model, paving the way for future development and scaling the unified multi-modal systems.

==> resources/math_macro.tex <==
\newcommand{\seedmoe}{Seed-MoE}

==> resources/packages.tex <==
% For flexible citation formats (author-year, numeric)
\usepackage{natbib}

% For UTF-8 encoded CJK (Chinese, Japanese, Korean) characters
\usepackage{CJKutf8}

% 允许使用 \newcommandx
\usepackage{xargs}  

% 用于创建 todo notes
\usepackage{todonotes}  

% 用于表格multirow
\usepackage{multirow}
\usepackage{booktabs}


% 用于cref
\usepackage{cleveref}

\usepackage{amsmath}
\usepackage{dsfont}

% % using itemize
% \usepackage{enumerate}


\usepackage{subcaption}


\usepackage{svg}

